March in Chat: Interactive Prompting for Remote Embodied Referring Expression

Many Vision-and-Language Navigation (VLN) tasks have been proposed in recent years, from room-based to object-based and indoor to outdoor. The REVERIE (Remote Embodied Referring Expression) is interesting since it only provides high-level instructions to the agent, which are closer to human commands in practice. Nevertheless, this poses more challenges than other VLN tasks since it requires agents to infer a navigation plan only based on a short instruction. Large Language Models (LLMs) show great potential in robot action planning by providing proper prompts. Still, this strategy has not been explored under the REVERIE settings. There are several new challenges. For example, the LLM should be environment-aware so that the navigation plan can be adjusted based on the current visual observation. Moreover, the LLM planned actions should be adaptable to the much larger and more complex REVERIE environment. This paper proposes a March-in-Chat (MiC) model that can talk to the LLM on the fly and plan dynamically based on a newly proposed Room-and-Object Aware Scene Perceiver (ROASP). Our MiC model outperforms the previous state-of-the-art by large margins by SPL and RGSPL metrics on the REVERIE benchmark.

==> section/algorithm.tex <==
\begin{algorithm}[t]
\small
\caption{March in Chat}\label{alg_integration}
\begin{algorithmic}
\State $I \gets \text{Instruction}$
\State $s_0 \gets \text{Initial state}$
%
\State $t \gets 0$  \Comment{Time step}
%

\While{k \textless \text{max step}}
    \State execute $a_{t}$
    
    \State $S_t \gets \text{Scene-Perceptor}(\text{current visual input})$
    \State $O\text{.insert}(O_t)$
    
    \If{current scene $S_t$ changes}
    \State $p_LLM = p(l|i,l)$
    \State $S \gets \text{(I,O,G)}$

    \EndIf
    
    \State $t \gets t+1$
    \State $a_{t} \gets \text{Action Prediction}(s)$
    

\EndWhile

\end{algorithmic}
\end{algorithm}

==> section/other_table.tex <==
\begin{table*}[!t]
\centering
\caption{Comparison with the state-of-the-art methods on REVERIE. SPL is the main metric for its navigation sub-task, and RGSPL is the main metric for the REVERIE task.}
\label{tab:reverie}
\vspace{-0mm}
\resizebox{\linewidth}{!}{
\begin{tabular}{l cccccc|cccccc|cccccc}
\toprule
\multicolumn{1}{l}{\multirow{3}{*}{Methods}} & \multicolumn{6}{c}{REVERIE Validation Seen} &\multicolumn{6}{c}{REVERIE Validation Unseen} & \multicolumn{6}{c}{REVERIE Test Unseen} \Tstrut\\
\cline{2-19}
~& \multicolumn{4}{c}{Navigation}  &  \multicolumn{1}{c}{\multirow{2}{*}{RGS$\uparrow$}}&
\multicolumn{1}{c|}{\multirow{2}{*}{RGSPL$\uparrow$}} & \multicolumn{4}{c}{Navigation}  & \multicolumn{1}{c}{\multirow{2}{*}{RGS$\uparrow$}}&
\multicolumn{1}{c|}{\multirow{2}{*}{RGSPL$\uparrow$}} & \multicolumn{4}{c}{Navigation}   & \multicolumn{1}{c}{\multirow{2}{*}{RGS$\uparrow$}}&
\multicolumn{1}{c}{\multirow{2}{*}{RGSPL$\uparrow$}}  \\
%\cline{2-5} \cline{8-11} \cline{14-17}  
~& \multicolumn{1}{c}{SR$\uparrow$} & \multicolumn{1}{c}{OSR$\uparrow$} & \multicolumn{1}{c}{SPL$\uparrow$}  & \multicolumn{1}{c}{TL} &  &  & \multicolumn{1}{c}{SR$\uparrow$} & \multicolumn{1}{c}{OSR$\uparrow$} & \multicolumn{1}{c}{SPL$\uparrow$} &\multicolumn{1}{c}{TL} & & & \multicolumn{1}{c}{SR$\uparrow$} & \multicolumn{1}{c}{OSR$\uparrow$} & \multicolumn{1}{c}{SPL$\uparrow$} & \multicolumn{1}{c}{TL} &  & \Tstrut\\

\midrule
Human & -- & --  & -- & {--} & -- & -- & -- & --  & --  & {--} & -- & -- & 81.51 & 86.83  & 53.66 &{21.18} & 77.84 &  51.44 \\
\midrule
RCM \cite{rcm} & 23.33 & 29.44 & 21.82& 10.70 & 16.23 & 15.36 & 9.29 & 14.23 & 6.97 &11.98 & 4.89 & 3.89 & 7.84 & 11.68 & 6.67 & 10.60 & 3.67 & 3.14\\
SMNA \cite{selfmonitor} & 41.25& 43.29  & 39.61& 7.54   & 30.07 &  28.98 & 8.15 & 11.28 &6.44 &9.07 & 4.54& 3.61 & 5.80& 8.39 & 4.53 & 9.23  & 3.10& 2.39 \\
FAST-Short \cite{fast} & 45.12& 49.68 &40.18&13.22  &31.41 & 28.11 & 10.08 & 20.48 & 6.17 &29.70 & 6.24 & 3.97 & 14.18 & 23.36 & 8.74 & 30.69  & 7.07 & 4.52 \\
FAST-MATTN \cite{reverie} &50.53 & 55.17 & 45.50 & 16.35&31.97 & 29.66 & 14.40 & 28.20 & 7.19 & 45.28  & 7.84 & 4.67 & 19.88 & {30.63} & 11.61 & 39.05 & 11.28 & 6.08 \\
ORIST~\cite{orist} & 45.19 & 49.12 & 42.21 & 10.73 & 29.87 & 27.77 & 16.84 & 25.02 & 15.14 & 10.90 & 8.52 & 7.58 & 22.19 & 29.20 & 18.97 & 11.38 & 10.68 & 9.28\\
RecBERT~\cite{recurrent} & 51.79 & 53.90 & 47.96& 13.44 & 38.23 & 35.61 &30.67 & 35.02 & 24.90 & 16.78 & 18.77 & 15.27 & 29.61 & 32.91 & 23.99 & 15.86 & 16.50 & 13.51 \\
AirBERT~\cite{airbert}& 47.01 & 48.98 & 42.34 & 15.16 & 32.75 & 30.01 & 27.89 & 34.51 & 21.88 & 18.71 & 18.23 & 14.18 & 30.28 & 34.20 & 23.61 & 17.91 & 16.83 & 13.28 \\
HAMT-ViT~\cite{hamt}&-&-&-&-&-&-&32.95&36.84&30.20&14.08&18.92&17.28&30.40&33.41&26.67&13.62&14.88&12.08\\
\midrule
HOP~\cite{hop}& 53.76 & 54.88 & 47.19 & 13.80 & 38.65 & 33.85 & 31.78 & 36.24 & 26.11 & 16.46 & 18.85 & 15.73 & 30.17 & 33.06 & 24.34 & 16.38 & 17.69 & 14.34\\
HOP+ & \textbf{55.87} & \textbf{56.43} & \textbf{49.55} & 10.59 & \textbf{40.76}& \textbf{36.22} & \textbf{36.07}& \textbf{40.04} & \textbf{31.13} & 14.57 & \textbf{22.49} & \textbf{19.33} & \textbf{33.82} & \textbf{35.81} & \textbf{28.24} & 15.17 & \textbf{20.20} & \textbf{16.86}  \\
\bottomrule
\end{tabular}}
\vspace{-0mm}
\end{table*}


\begin{figure}[t]
    \centering
    \scriptsize
      \renewcommand{\tabcolsep}{1.0mm}
    \begin{tabular}{l|rl}
    \toprule
         \multirow{4}{*}{\STAB{\rotatebox[origin=c]{90}{\sc Object}}}& 
         \textbf{Task:} & Turn on the washing machine  \\
         &\textbf{Goal:}& The target object is: \\
         &\textbf{Answer:}& washing machine \\
         \midrule
         \multirow{5}{*}{\STAB{\rotatebox[origin=c]{90}{\sc Place}}}& 
         \multicolumn{2}{l}{I am a question-answering bot. If you ask me a question, I will give you the answer.}\\
         %\\
         &\textbf{Question:}& Where does a microwave can usually appear in a house? \\
         &\textbf{Answer:}& kitchen.\\
         &\textbf{Question:}& Where does a \textbf{washing machine} can usually appear in a house?\\
         &\textbf{Answer:}& laundry room.\\
         \bottomrule
    \end{tabular}
    \caption{Examples of prompting template}
    \vspace{-0.2in}
    \label{fig:thinker}
\end{figure}


\begin{table}[!t]
    \centering
    \scriptsize
      %
    \begin{tabular}{l}
    \toprule 
         \textbf{R2R}\\
         Go up the stairs and then walk the length of the couch.  Walk past the dining\\
         area and into the kitchen.  Stop in front of the refrigerator.\\
         \midrule
         \textbf{FGR2R} \\
         Step 1: go up the stair  \\
         Step 2: and then walk the length of the couch \\
         Step 3: walk past the dining area and into the kitchen\\
         Step 4: stop in front of the refrigerator\\         
         %\midrule
         \bottomrule
    \end{tabular}
    \caption{Instruction example of R2R and FGR2R}
    \vspace{-0.2in}
    \label{fig:fgr2r}
\end{table}


